Riemannian Walk for Incremental Learning: Understanding Forgetting and Intransigence

Incremental learning (IL) has received a lot of attention recently, however, the literature lacks a precise problem definition, proper evaluation settings, and metrics tailored specifically for the IL problem. One of the main objectives of this work is to fill these gaps so as to provide a common ground for better understanding of IL. The main challenge for an IL algorithm is to update the classifier whilst preserving existing knowledge. We observe that, in addition to forgetting, a known issue while preserving knowledge, IL also suffers from a problem we call intransigence, inability of a model to update its knowledge. We introduce two metrics to quantify forgetting and intransigence that allow us to understand, analyse, and gain better insights into the behaviour of IL algorithms. We present RWalk, a generalization of EWC++ (our efficient version of EWC [Kirkpatrick2016EWC]) and Path Integral [Zenke2017Continual] with a theoretically grounded KL-divergence based perspective. We provide a thorough analysis of various IL algorithms on MNIST and CIFAR-100 datasets. In these experiments, RWalk obtains superior results in terms of accuracy, and also provides a better trade-off between forgetting and intransigence.

==> analysis.tex <==
\section{Analysis}

\begin{figure}[thpb]
\centering
\includegraphics[scale=0.45]{../plots/mnist_scatter_plot.pdf}
\caption{Combined comparison }
\label{fig:mnist_scatter}
\end{figure}


\begin{figure}[thpb]
\begin{center}
\begin{subfigure}{0.40\linewidth}
\begin{center}
\includegraphics[scale=0.40]{../plots/mnist_sampling_acc_abal.pdf}
\end{center}
\end{subfigure}%
\begin{subfigure}{0.40\linewidth}
\begin{center}
\includegraphics[scale=0.40]{../plots/mnist_sampling_fgt_abal.pdf}
\end{center}
\end{subfigure}
\end{center}
\caption{\em Comparison of different sampling strategies in our method on MNIST. The plots are generated on MNIST with ($\lambda, \eta, \alpha$) set to ($1$, $0.1$, $0.9$). Average accuracy (left), Forgetting Measure(Right)}
\label{fig:mnist_sampling_comp}
\end{figure}

\begin{figure}[thpb]
\begin{center}
\begin{subfigure}{0.40\linewidth}
\begin{center}
\includegraphics[scale=0.40]{../plots/cifar_sampling_acc_abal.pdf}
\end{center}
\end{subfigure}%
\begin{subfigure}{0.40\linewidth}
\begin{center}
\includegraphics[scale=0.40]{../plots/cifar_sampling_fgt_abal.pdf}
\end{center}
\end{subfigure}
\end{center}
\caption{\em Comparison of different sampling strategies in our method on CIFAR-100. The plots are generated on CIFAR-100 with ($\lambda, \eta, \alpha$) set to ($10$, $0.001$, $0.3$). Average accuracy (left), Forgetting Measure(Right)}
\label{fig:mnist_sampling_comp}
\end{figure}

\ajcomment{Just discussing whatever coming into my mind. Please put it in the
text in a coherent form and cut it short.} 

Note that, from
Table~\ref{tab:comp_with_baslines} and Figs.~\ref{fig:mnist_acc} 
and~\ref{fig:cifar_acc}, it is clear that our algorithm is the best 
performing in terms of average accuracy on both the datasets, except for MNIST without
sampling in which PI is slightly better. The high accuracy of PI is mainly
influenced by preserving knowledge on task 1 (top left in
Fig.~\ref{fig:mnist_acc}). However, with samples, even though the accuracy of
all the methods improved, our method clearly outperforms all other methods
($~5\%$ better on MNIST) while maintaining very low forgetting measure. The
importance of having even a small number of samples dramatically improve the
intransigence measure as shown in Fig.~\ref{fig:nl}. This clearly shows the
inability of the methods to differentiate the current classes from the
previously learned classes in the absence of previous samples.

Note that, as mentioned in Section~\ref{sec:measures}, evaluating incremental
learners in not trivial. In fact, after training for all the tasks, measuring
the standard multi-class accuracy does not truly evaluate the merits of an
incremental learning system. For example, two methods that have similar average
accuracy may have different forgetting and intransigence measures. In fact,
forgetting and intransigence measures are negatively correlated. For instance,
vanilla has the best intransigence measure as it has full flexibility to learn
the new task while forgetting on the previous tasks completely. Adding
regularization improves forgetting with a trade-off of not learning in the new
task. Therefore, the ideal incremental learning algorithm should be able to
learn on the new task as good as vanilla with minimal forgetting on the previous
tasks. We show different algorithms in a scatter plot in
Fig.~\ref{fig:mnist_scatter} where the two axes are forgetting and
intransigence, to accurately measure their performance. Here, the ideal
algorithm should be in the bottom-left corner. Note that, our algorithm with
samples is the best performing next to PI with sampling. Furthermore, having only $10$
samples per class on MNIST, the intransigence measure improved dramatically for
all the methods and our method is the best in preserving forgetting measure. We
believe, with our measures incremental learning algorithms can be accurately
evaluated which would be useful to design better algorithms.


In Fig.~\ref{fig:mnist_sampling_comp}, we show the performance of our method
with different sampling strategies. In this a naive uniform sampling approach
performs as good as an intelligent plane distance based and iCaRL based
sampling. This may be due to the simplicity of the MNIST dataset\ajcomment{any
other reason?}


==> prelim.tex <==

\section{Preliminaries}
\label{sec:prelim}
We first briefly review the probabilistic interpretation of neural networks
and an approximate form of the KL-divergence both of which are crucial to our
approach.

%\vspace{-2ex}
\subsubsection{Probabilistic Interpretation of Neural Networks}
In a probabilistic sense, for a classification
task, a neural network models a discrete conditional probability distribution
of the form $p_{\param}(\op | \ip)$ (usually the softmax output), where $\ip$ is the
input and $\param$ are the network parameters (for simplicity, we will use
$p_{\param}$ and $p_{\param}(\op | \ip)$ interchangeably). The prediction label $\hat{y}$ can then be obtained by sampling from a multinoulli distribution, $t(y) = \prod_{j=1}^K p_{\param,j}^{[y=j]}$, where $p_{\param,j}$ is the probability of the $j$-th class, $K$ are the total number of classes in the dataset, and $[\cdot]$ is Iverson bracket. Note that $t(y)$ is defined by $p_{\param}$ and sampling from it yield a single label/ prediction. Typically, instead of doing such sampling, a label with the highest probability $p_{\param}$ is chosen as the output of the network. 


%%or
%%by taking the label with the highest probability.
% The prediction label $\hat{y}$ can then be obtained by sampling
% over the multinoulli distribution (for multi-label classification) defined by
% the discrete conditional distribution $p_{\param}(\op | \ip)$. Instead of
% sampling, the standard approach is to consider the label with the highest
% probability as the final prediction.  

%\vspace{-2ex}
\subsubsection{Approximation of KL-divergence}\label{sec:kl}
The similarity between any two distributions can be measured
using the KL-divergence~\cite{Kullback51KLdivergence}. Let $\KL(p_{\param}
\| p_{\param + \Delta \param})$ be the KL-divergence between probability
distributions defined by the parameters $\param$ and $\param + \Delta \param$.

\begin{lemma}\label{lem:klapprox}
\label{lemma:kl_approx}
Assuming $\Delta \param \to 0$, the second-order Taylor approximation of
KL-divergence can be
written~\cite{Amari98NaturalGradient,Pascanu14NaturalGradient} as:
\vspace{-2ex}
\begin{equation}
\label{eq:KLapprox_prelim}
    \KL(p_{\param} \| p_{\param + \Delta \param}) \approx
     \frac{1}{2} \Delta \param^{\top} F_{\param} \Delta \param\ , \footnote{proof is given in the supplementary material}
     %\vspace{-2ex} 
\end{equation}
where $F_{\param}$ is the empirical Fisher at $\param$.
\end{lemma}

Before explaining the empirical version of a Fisher information matrix, we will first define it in its true form:

\SKIP{Let us now describe an approximation of KL-divergence when $\Delta \param \to
0$, which is crucial to our approach.
For this, we first we define the Fisher information matrix.}

\begin{definition}{Fisher}
\label{dfn:fisher}
Let $p_{\param}(\op|\ip)$ be a probability distribution defined by the
parameters $\param$. The Fisher information matrix at $\param$ can be
defined~\cite{Amari98NaturalGradient} as:
%\vspace{-2ex}
\begin{equation}\label{eq:fisher}
\tilde{F}_{\param} = \E_{\ip \sim \dataset, \op \sim p_{\theta}(\op | \ip)}
\left[\left( \frac{\partial \log p_{\param}( \op | \ip) }{\partial \param} \right) \left( \frac{\partial \log
p_{\param}( \op | \ip) }{\partial \param} \right)^{\top}\right] \ ,
%\vspace{-2ex}
\end{equation}
where $\dataset$ is the dataset.
\end{definition}

Note that computing this Fisher matrix requires computing gradients using
labels sampled from the model distribution $p_{\theta}(\op | \ip)$, which
requires multiple backward passes (more details are given in the supplementary).
Thus, for efficiency, Fisher is often replaced with an empirical
Fisher~\cite{martens2016second}, where the expectation is taken over the
data distribution, \ie, both $\ip$ and $\op$ are now sampled from $\dataset$, and we use this to
approximate the KL.
%
%We are now ready to write the approximation of KL-divergence.

From the Lemma~\ref{lemma:kl_approx}, it can be seen that when $\Delta \param \to 0$,
$\KL(p_{\param} \| p_{\param + \Delta \param})$ behaves like a distance
measure. Therefore, the mapping $\manifold$ from the parameters $\param\in
\real^\paramdim$ to the probability densities $p_{\param}$ defines a Riemannian
manifold\footnote{A Riemannian manifold is a real smooth manifold equipped with
an inner product on the tangent space at each point that varies smoothly from
point to point~\cite{lee2006riemannian}.}, where the Fisher matrix $F_{\param}$ defines the distance
metric. Note that, the distance metric in Riemannian manifold has to be positive definite, but $F_{\theta}$
is positive semi-definite~\cite{martens2016second}. This makes it a
pseudo-manifold.

Note that, the matrix $F_{\theta} $ is of size $\paramdim \times \paramdim$,
which is infeasible to store given the number of parameters in neural networks are
normally in the order of millions. Thus, similarly
to~\cite{Kirkpatrick2016EWC}, we assume parameters to be independent of each
other which results in the diagonal approximation of $F_{\param}$. Thus,
Eq.~(\ref{eq:KLapprox_prelim}) can be written as:
%\vspace{-2ex}
\begin{equation}\label{eq:klapproxdiag1}
\KL(p_{\param} \| p_{\param + \Delta \param}) \approx
\frac{1}{2} \sum_{i=1}^{\paramdim} F_{\theta_i}\, \Delta \param_i^2\ ,
%\vspace{-1ex}
\end{equation}
%\vspace{-1.5ex}
where $\param_i$ is the $i$-th entry of the parameter vector $\param$.



\SKIP{
It is well known that, in its infinitesimal form, KL divergence can be
interpreted as a distance
measure~\cite{Amari98NaturalGradient,Pascanu14NaturalGradient}
(Lemma~\ref{lem:klapprox}) in the Riemannian manifold induced by the Fisher
information matrix $F_{\param}$. Every $\param\in \real^\paramdim$ maps to a
probability density in the manifold where the Fisher matrix defines the
similarity measure or the norm between them.

%Let us define our functional manifold $\manifold$ be a mapping from the
%parameters $\param\in \real^\paramdim$ to the probability densities
%$p_{\param}$. 
%Hence, $\manifold$ defines a Riemannian manifold where KL divergence between nearby
%density functions defines the similarity measure.  
%\begin{lemma}\label{lem:klapprox}
%Assuming $\Delta \param \to 0$, the second order Taylor approximation of KL-divergence can
%be written as,
%\begin{equation}
%\label{eq:KLapprox}
%    \KL(p_{\param} \| p_{\param + \Delta \param}) \approx
%     \frac{1}{2} \Delta \param^{\top} (F_{\param} + \eta I)\, \Delta \param\ , 
%\end{equation}
%where $F_{\param} = \E_{\ip \sim p_d, \op \sim p_{\theta}(\op | \ip)} \left[\left( \frac{\partial \log
%p_{\param}( \op | \ip) }{\partial \param} \right) \left( \frac{\partial \log
%p_{\param}( \op | \ip) }{\partial \param} \right)^{\top}\right]$ is
%the Fisher information matrix at $\param$, $\eta \in \real$, $p_d$ is the data distribution, and $I$ is the identity matrix.
%\end{lemma}
\begin{lemma}\label{lem:klapprox}
Assuming $\Delta \param \to 0$, the second order Taylor approximation of KL-divergence can
be written as,
\begin{equation}
\label{eq:KLapprox}
    \KL(p_{\param} \| p_{\param + \Delta \param}) \approx
     \frac{1}{2} \Delta \param^{\top} F_{\param} \Delta \param\ , 
\end{equation}
where $F_{\param} = \E_{\ip \sim p_d, \op \sim p_{\theta}(\op | \ip)} \left[\left( \frac{\partial \log
p_{\param}( \op | \ip) }{\partial \param} \right) \left( \frac{\partial \log
p_{\param}( \op | \ip) }{\partial \param} \right)^{\top}\right]$ is
the Fisher information matrix at $\param$ and $p_d$ is the data
distribution.
\end{lemma}

Since taking the expectation over $p_{\theta}$ would require multiple forward
passes, the standard approach is to resort to the empirical Fisher, where the
expectations are taken over $\ip$ and $\op$ from the ground truth data. Note
that, at a minimum, the predictions are as good as the ground truth labels, \ie,
gradients are nearly zero, thus, the Fisher becomes nearly zero. To avoid this,
we use $F_{\theta} + \eta I$ where $\eta \in \R$ is a hyperparameter and $I$ is
the identity matrix.
More precisely, adding $\eta$ approximates Fisher
to the Hessian\footnote{By Hessian, we mean the expected value of Hessian of
$-\log p_{\param}$.} at the minimum where the constant curvature is captured
by $\eta$.
}



%This equation is used to approximate KL divergence in our approach.
%Now, let us explain the KL divergence based regularization which is a key
%component of our loss function.

